Exciton spectrum in atomically thin monolayers: The role of hBN encapsulation

The high-quality structures containing semiconducting transition metal dichalcogenides (S-TMDs) monolayer (MLs) required for optical and electrical studies are achieved by their encapsulation in hexagonal BN (hBN) flakes. To examine the effect of hBN thickness in these systems, we consider a model with an S-TMD ML placed between a semi-infinite in the out-of-plane direction substrate and complex top cover layers: a layer of finite thickness, adjacent to the ML, and a semi-infinite in the out-of-plane direction top part. We obtain the expression for the Coulomb potential for such a structure. Using this result, we demonstrate that the energies of excitonic $s$ states in the structure with WSe$_2$ ML change significantly for the top hBN with thickness less than 30 layers for different substrate cases, such as hBN and SiO$_2$. For the larger thickness of the top hBN flake, the binding energies of the excitons are saturated to their values of the bulk hBN limit.

==> final arxiv/SI_CLEAN.tex <==
	\begin{center}
	%%%%%%%%% ABSTRACT TITLE
	{\large Supplementary Material for "Exciton spectrum in atomically thin monolayers: \\ 	The role of hBN encapsulation"}
	%%%%%%%%% ABSTRACT AUTHORS
\end{center}


\section{The modified Rytova-Keldysh potential for the case of ultrathin top hBN flake}

In our study, we modeled the top layer of hBN with its thickness $L$ and the macroscopic in- ($\varepsilon_{\text{hBN},\parallel}$) and out-of-plane ($\varepsilon_{\text{hBN},\perp}$) dielectric constants of hBN, $i.e.$, in the limit of the continuous hBN medium.  
However, in the case of the ultrathin top hBN flake, where it consists of only a few layers of hBN monolayers, the use of such a limit is doubtful. 
In order to find the limits of applicability of the continuous model, we derive the modified Rytova-Keldysh potential with a few layers of the hBN. 

To do it, we consider the modification of the system studied in the main text. 
The bottom semi-infinite substrate remains unchanged.
Thus, it is characterized by in- ($\varepsilon_{1,\parallel}$) and out-of-plane ($\varepsilon_{1,\perp}$) dielectric constants and occupies the domain $z\in]-\infty, -\delta]$. 
The S-TMD monolayer is placed in the plane $z=0$ with its in-plane polarizability $\chi_\text{TMD}$. 
The first top hBN flake consists of $N$ layer and has a thickness $L=Nd$. 
Here $d=0.33$\, nm is the distance between the hBN layers in a bulk hBN crystal. 
The $j$th layer of the hBN flake is placed in the $z_j=jd$ plane. 
Each hBN layer is characterized by the in-plane polarizability $\chi_\text{hBN}$. 
The second top layer with the in- ($\varepsilon_{3,\parallel}$) and out-of-plane ($\varepsilon_{3,\perp}$) dielectric constants occupies the domain $z\in[L+\delta, \infty[$. 

In order to find the potential energy between two charges in the S-TMD monolayer, we solve the following electrostatic problem.
We consider the point-like charge $Q$ at the point $(0,0,z')$, where $0<z'\neq z_j <L$ and calculate the potential in such a system following~\cite{Cudazzo2011}.
Similarly to the previous case, we consider 3 regions: bottom semi-infinite medium with the potential
$\Phi_1(\boldsymbol{\rho},z)$, second top semi-infinite layer with the potential $\Phi_3(\boldsymbol{\rho},z)$, 
and the space between them with the potential $\Phi_2(\boldsymbol{\rho},z)$, where we introduced the in-plane 
vector $\boldsymbol{\rho}=(x,y)$.
Using the cylindrical symmetry of the problem, we present the potentials in the form
\begin{equation}
\label{eq:fourier}
\Phi_j(\boldsymbol{\rho},z)=\frac{1}{(2\pi)^2}\int d^2\mathbf{k} e^{i\mathbf{k}\boldsymbol{\rho}}\Phi_j(\mathbf{k},z)
\end{equation}

The Maxwell's equation $\text{div}\,\mathbf{D}_{1,3}=0$ for 1-st and 3-rd regions ($j=1,3$) reads
\begin{equation}
-\varepsilon_{j,\parallel}\mathbf{k}^2\Phi_{j}(\mathbf{k},z)+\varepsilon_{j,\perp}\frac{d^2\Phi_j(\mathbf{k},z)}{dz^2}=0.
\end{equation}
The solutions to these equations are
\begin{align}
\Phi_1(\mathbf{k},z)&=Ae^{\kappa_1 z},  &\text{for}& \, z\in]-\infty,-\delta] , \\
\Phi_3(\mathbf{k},z)&=Be^{-\kappa_3 z}, &\text{for}& \, z\in [L+\delta, \infty[,
\end{align}
where $\kappa_j=|\mathbf{k}|\sqrt{\varepsilon_{j,\parallel}/\varepsilon_{j,\perp}}=
k\sqrt{\varepsilon_{j,\parallel}/\varepsilon_{j,\perp}}$.

The equation for the potential $\Phi_2(\mathbf{r},z)$ takes the form
\begin{align}
\label{eq:second_potential}
\Delta_\parallel\Phi_2(\boldsymbol{\rho},z)+&\epsilon_\perp\frac{d^2\Phi_2(\boldsymbol{\rho},z)}{dz^2}= \nonumber \\ &-4\pi[Q\delta(\boldsymbol{\rho})\delta(z-z') - \varrho_\text{ind}(\boldsymbol{\rho},z)],
\end{align}
where $\Delta_\parallel$ is 2D Laplace operator. 
We introduced the out-of-plane dielectric constant ($\epsilon_\perp$) of the hBN flake with $N>1$. 
In the case $N=1$, one needs to put $\epsilon_\perp=1$.   
The first term on the right-hand side of the equation is the charge density of the charge $Q$.
The second term $\varrho_\text{ind}(\boldsymbol{\rho},z)$ represents the induced charge density
due to the polarization of the hBN and S-TMD layer by charge $Q$.
Following Ref.~\cite{Cudazzo2011}, we present the induced charge in the form
\begin{align}
\varrho_\text{ind}(\boldsymbol{\rho},z)=-&\chi_\text{hBN}\sum_{j=1}^N \delta(z-z_j)\Delta_\parallel\Phi_2(\boldsymbol{\rho},z_j)-
\nonumber \\ -&\chi_\text{TMD}\delta(z)\Delta_\parallel\Phi_2(\boldsymbol{\rho},0).
\end{align}
Using the Fourier transform (\ref{eq:fourier}) of the potential $\Phi_2(\boldsymbol{\rho},z)$ 
we present Eq.~(\ref{eq:second_potential}) as 
\begin{align}
\label{eq:second_potential_k}
\Big[\mathbf{k}^2-\epsilon_\perp\frac{d^2}{dz^2}\Big]\Phi_2(\mathbf{k},z)=&4\pi Q\delta(z-z')-
2r_0k^2\delta(z)\Phi_2(\mathbf{k},0) \nonumber \\
-&2R_0k^2\sum_{j=1}^N\delta(z-z_j)\Phi_2(\mathbf{k},z_j),
\end{align}
where we introduced the in-plane screening lengths $r_0=2\pi\chi_\text{TMD}$ and $R_0=2\pi\chi_\text{hBN}$ for 
S-TMD and hBN monolayers, respectively.
Integrating this equation in the regions $z\in[-\epsilon, \epsilon]$, $z\in[z_j-\epsilon, z_j+\epsilon]$, and $z\in[z'-\epsilon,z'+\epsilon]$ one obtains the following conditions in the limit $\epsilon\rightarrow 0$
\begin{align}
\epsilon_\perp\frac{d\Phi_2(\mathbf{k},z)}{dz}\Big|^{+0}_{-0}&=2r_0k^2\Phi_2(\mathbf{k},0), \\
\epsilon_\perp\frac{d\Phi_2(\mathbf{k},z)}{dz}\Big|^{z_j+0}_{z_j-0}&=2R_0k^2\Phi_2(\mathbf{k},z_j),\\
\epsilon_\perp\frac{d\Phi_2(\mathbf{k},z)}{dz}\Big|^{z'+0}_{z'-0}&=-4\pi Q.
\end{align} 
At the points $z\neq 0\,,z_j\,,z'$ the Eq.~(\ref{eq:second_potential_k}) is simplified
\begin{equation}
\Big[\mathbf{k}^2-\epsilon_\perp\frac{d^2}{dz^2}\Big]\Phi_2(\mathbf{k},z)=0
\end{equation}
Therefore, the general solution for $\Phi_2(\mathbf{k},z)$ can be written in the form
\begin{align}
\label{eq:potential2}
\Phi_2(\mathbf{k},z)=&\Psi_0e^{-K|z-z'|}+\sum_{j=1}^N \Psi_je^{-K|z-z_j|} + 
\nonumber \\ +&
\Psi e^{-K|z|}+ \alpha e^{Kz} +\beta e^{-Kz},
\end{align}
where $\Psi_0$,$\Psi_j$,$\Psi$, $\alpha$ and $\beta$ are unknown functions of $K=k/\sqrt{\epsilon_\perp}$.
The aforementioned boundary conditions together with the equation give the following restrictions
\begin{align}
\label{eq:boundary_conditions}
\Psi=&-r_0K\Phi_2(\mathbf{k},0), \nonumber \\
\Psi_j=&-R_0K\Phi_2(\mathbf{k},z_j), \nonumber \\
\Psi_0=&2\pi Q/\epsilon_\perp K.
\end{align}
Considering the boundary conditions for the electrostatic potential and for the out-of-plane component of the displacement field 
 at $z=-\delta$ 
\begin{align}
\Phi_1(\mathbf{k},-\delta)&=\Phi_2(\mathbf{k},-\delta), \\ \frac{\varepsilon_{1,\perp}}{\epsilon_\perp}
\frac{d\Phi_1(\mathbf{k},z)}{dz}\Big|_{z=-\delta}&=\frac{d\Phi_2(\mathbf{k},z)}{dz}\Big|_{z=-\delta},
\end{align}
and at $z=L+\delta$
\begin{align}
\Phi_3(\mathbf{k},L+\delta)&=\Phi_2(\mathbf{k},L+\delta), \\  \frac{\varepsilon_{3,\perp}}{\epsilon_\perp}
\frac{d\Phi_3(\mathbf{k},z)}{dz}\Big|_{z=L+\delta}&=\frac{d\Phi_2(\mathbf{k},z)}{dz}\Big|_{z=L+\delta},
\end{align}
we get the following equations
\begin{widetext}
\begin{align}
&Ae^{-\kappa_1\delta}=\Psi_0e^{-K(z'+\delta)}+\sum_{j=1}^N\Psi_je^{-K(z_j+\delta)}+\Psi e^{-K\delta}+\alpha e^{-K\delta}+\beta e^{K\delta}, \\
&A\frac{\varepsilon_1}{\sqrt{\epsilon_\perp}}e^{-\kappa_1\delta}=\Psi_0e^{-K(z'+\delta)}+\sum_{j=1}^N\Psi_je^{-K(z_j+\delta)}+
\Psi e^{-K\delta}+\alpha e^{-K\delta}-\beta e^{K\delta}, \\
&Be^{-\kappa_3 (L+\delta)}=\Psi_0e^{-K(L+\delta-z')}+\sum_{j=1}^N\Psi_je^{-K(L+\delta-z_j)}+\Psi e^{-K(L+\delta)}+
\alpha e^{K(L+\delta)}+\beta e^{-K(L+\delta)},  \\
&B\frac{\varepsilon_3}{\sqrt{\epsilon_\perp}}e^{-\kappa_3 (L+\delta)}=\Psi_0e^{-K(L+\delta-z')}+\sum_{j=1}^N\Psi_je^{-K(L+\delta-z_j)}+\Psi e^{-K(L+\delta)}-\alpha e^{K(L+\delta)}+\beta e^{-K(L+\delta)}. 
\end{align}
\end{widetext}
where we introduced the short notation $\varepsilon_j=\sqrt{\varepsilon_{j,\perp}\varepsilon_{j,\parallel}}$ for $j=1,3$.
Introducing $a=\varepsilon_1/\sqrt{\epsilon_\perp}$ and $b=\varepsilon_3/\sqrt{\epsilon_\perp}$, and considering the general case $a,b\neq 1$ we remove the parameters $A$ and $B$ from the above equations and obtain
\begin{widetext}
\begin{align}
\Psi_0e^{-K(z'+\delta)}+\sum_{j=1}^N\Psi_je^{-K(z_j+\delta)}+\Psi e^{-K\delta}+\alpha e^{-K\delta}+\Big(\frac{a+1}{a-1}\Big)\beta e^{K\delta}=0,\\
\Psi_0e^{-K(L+\delta-z')}+\sum_{j=1}^N\Psi_je^{-K(L+\delta-z_j)}+\Psi e^{-K(L+\delta)}+\Big(\frac{b+1}{b-1}\Big)\alpha e^{K(L+\delta)}+
\beta e^{-K(L+\delta)}=0. 
\end{align}
\end{widetext}
 
Note that the solution of the aforementioned system of equations for the case $a=1$ and/or $b=1$ can be obtained
from the general solution by taking the corresponding limit. 

We solve the general equation in a few steps. 
First, we write the system of equations in the following form
\begin{align}
\label{eq:alphabeta}
e^{-K\delta}\alpha+\Big(\frac{a+1}{a-1}\Big)e^{K\delta}\beta=&\mathcal{A}, \nonumber  \\
\Big(\frac{b+1}{b-1}\Big)e^{K(L+\delta)}\alpha+e^{-K(L+\delta)}\beta=&\mathcal{B},
\end{align}
where we introduced the following notations $\mathcal{A}=-\Psi_0e^{-K(z'+\delta)}-\sum_{j=1}^N\Psi_je^{-K(z_j+\delta)}-\Psi e^{-K\delta}$, 
$\mathcal{B}=-\Psi_0e^{-K(L+\delta-z')}-\sum_{j=1}^N\Psi_je^{-K(L+\delta-z_j)}-\Psi e^{-K(L+\delta)}$.
Solving the system of equations (\ref{eq:alphabeta}) one gets
\begin{align}
\alpha=\frac{\mathcal{A}e^{-K(L+\delta)}-\mathcal{B}\Big(\frac{a+1}{a-1}\Big)e^{K\delta}}{D}, \\
\beta=\frac{\mathcal{B}e^{-K\delta}-\mathcal{A}\Big(\frac{b+1}{b-1}\Big)e^{K(L+\delta)}}{D}, 
\end{align}
with $D=e^{-K(L+2\delta)}-\Big(\frac{a+1}{a-1}\Big)\Big(\frac{b+1}{b-1}\Big)e^{K(L+2\delta)}$.
Substituting these solutions into (\ref{eq:potential2}), we express $\Phi_2(\mathbf{k},z)$ via $N+2$ parameters $\Psi_0$, $\Psi_j$ and $\Psi$. 
Then, using the latter expression, we calculate the expressions for the potential in $z=0$,  $z=z'$, and $z=z_l,\, l=1,2\dots N$ points
\begin{widetext}
\begin{align}
\label{eq:self_consisted}
\Phi_2(\mathbf{k},0)=&\Psi_0e^{-Kz'}+\sum_{j=1}^N\Psi_je^{-K z_j }+\Psi+\alpha+\beta, \nonumber \\
\Phi_2(\mathbf{k},z')=&\Psi_0+\sum_{j=1}^N \Psi_je^{-K(z_l-z')} + \Psi e^{-K z'}+ \alpha e^{Kz'} +\beta e^{-Kz'},\nonumber  \\
\Phi_2(\mathbf{k},z_l)=&\Psi_0e^{-K(z_l-z')}+\sum_{j=1}^N \Psi_je^{-K|z_l-z_j|} + \Psi e^{-Kz_l}+ \alpha e^{Kz_l} +\beta e^{-Kz_l},
\end{align}
\end{widetext}
which together with (\ref{eq:boundary_conditions}) gives the complete set of equations for the parameters 
$\Psi_0$, $\Psi_j$, and $\Psi$. 
In the system of Eqs.~(\ref{eq:self_consisted}), we considered the particular case $0<z'<z_1<z_2<\dots < z_N=L$ for simplicity. Then we simplify our solutions by taking the following limits $\delta\rightarrow 0$ and $z'\rightarrow 0$, and obtain $\Phi_2(\mathbf{k},z=0)=(2\pi Q/k)v(k)$ which defines the electrostatic potential $\Phi(\rho)$ in the S-TMD plane, which reads
\begin{align}
\Phi(\rho)=Q\int_0^\infty dk J_0(k\rho)v(k). 
\end{align}
We derive the expressions for the case of monolayer ($v_\text{m}$) and bilayer ($v_\text{b}$) hBN flake to demonstrate
the aforementioned algorithm and then estimate the spectrum of excitons for both cases.   

First, we consider the case of monolayer hBN, $i.e.$, $N=1$, $\epsilon_\perp=1$, and hence $a=\varepsilon_1$, $b=\varepsilon_3$ and $K=k$. 
Following the procedure mentioned above, we obtain the result for the monolayer (m) 
\begin{align}
v_\text{m}(k)=
\frac{1-\left(\frac{2kR_0+\varepsilon_3-1}{2kR_0+\varepsilon_3+1}\right)e^{-2dk} }{(kr_0+\frac{\varepsilon_1+1}{2})-
(kr_0+\frac{\varepsilon_1-1}{2})\left(\frac{2kR_0+\varepsilon_3-1}{2kR_0+\varepsilon_3+1}\right)e^{-2dk}}.
\end{align}
Note that this result looks similar to the general result in the main text (see Eq.~23).
The eigenvalue problem for this potential has a form 
\begin{align}
\Big[\widetilde{b}^2\frac{1}{\xi}\Big(\xi\frac{d}{d\xi}\Big)+2\widetilde{b}\int_0^\infty dx J_0(x\xi)v_\text{m}(x)+\epsilon\Big]\psi(\xi)=0.
\end{align}
Here $v_\text{m}(x=kr_0)\equiv v_\text{m}(k)$, $\epsilon=E/Ry$ and $\xi=\rho/r_0$ are the dimensionless energy and coordinate, respectively, with $Ry=\mu e^4/2\hbar^2$ and $\widetilde{b}=\hbar^2/(\mu e^2r_0)$. 
To calculate the spectrum of excitons, we consider the particular case $\varepsilon_1=\varepsilon_\text{hBN}=4.5$,
$\varepsilon_3=1$. 
Using formula (4) from Ref.~\cite{Berkelbach2013} and in-plane dielectric constant of the monolayer hBN 
$\varepsilon_{\text{hBN},\parallel}=4.98$ from \cite{Laturia2018} 
$R_0=(\varepsilon_{\text{hBN},\parallel}-1)d/2$, we obtain $R_0=6.57\,\mbox{\AA}$. 
Note that this screening length is much smaller than, for example, in the WSe$_2$ monolayer $r_0=45\,\mbox{\AA}$ \cite{Berkelbach2013}. 
Solving the eigenvalue equation with $\widetilde{b}\approx 0.056$ and taking into account that $Ry=2.856$\,eV we obtain the following binding energies: $E_1\approx -246$\,meV, $E_2\approx -75$\,meV, $E_3\approx-36$\,meV, $E_4\approx-21$\,meV, $E_5\approx-14$\,meV.
Note that this result is close to the result of the homogeneous model proposed in the main text:  
$E_1\approx -235$\,meV, $E_2\approx -73$\,meV, $E_3\approx-36$\,meV, $E_4\approx-21$\,meV, $E_5\approx-14$\,meV.
The main difference between the two calculated spectra is the binding energy of the $1s$ exciton. 
The smaller binding energy of the $1s$ state in the homogeneous model can be explained by the less effective screening of the Coulomb potential than in the model considered here.    
 
The potential for the case of the bilayer flake $N=2$ $\Phi_2(\mathbf{k},z=0)=(2\pi Q/k\sqrt{\epsilon_\perp})v_\text{b}(k)$ 
with the corresponding out-of-plane dielectric constant $\epsilon_\perp$ is 
\begin{widetext}
\begin{align}
v_\text{b}(k)=\frac{1-\frac{2KR_0(b+2KR_0)}{(KR_0+1)(b+2KR_0+1)}e^{-2dK} +\frac{(KR_0-1)(b+2KR_0-1)}{(KR_0+1) (b+2KR_0+1)}e^{-4dK}}{\frac{a+1}{2}+Kr_0-\frac{[(a+2Kr_0) (b+2KR_0)-1]}{(KR_0+1)(b+2KR_0+1)}KR_0e^{-2dK}+\frac{(KR_0-1) (b+2KR_0-1)}{(KR_0+1)(b+2KR_0+1)}\left(\frac{a-1}{2}+Kr_0\right) e^{-4dK}}.
\end{align}
\end{widetext}
Here $K=k/\sqrt{\epsilon_\perp}$, $a=\varepsilon_1/\sqrt{\epsilon_\perp}$, and $b=\varepsilon_3/\sqrt{\epsilon_\perp}$.
The eigenvalue problem for the case of the bilayer reads 
\begin{align}
\Big[\widetilde{b}^2\epsilon_\perp\frac{1}{\xi}\Big(\xi\frac{d}{d\xi}\Big)+2\widetilde{b}\int_0^\infty dx J_0(x\xi)
v_\text{b}(x)+\epsilon\Big]\psi(\xi)=0.
\end{align}
Here $v_\text{b}(x=kr_0/\sqrt{\epsilon_\perp})\equiv v_\text{b}(k)$, $\epsilon=E/Ry$ and
$\xi=\rho\sqrt{\epsilon_\perp}/r_0$ are the dimensionless energy and coordinate, 
respectively, with $Ry=\mu e^4/2\hbar^2$ and $\widetilde{b}=\hbar^2/(\mu e^2r_0)$. 
For the numerical estimation of the exciton spectrum in this case, we use $\varepsilon_1=4.5$ and $\varepsilon_3=1$ and the result of Ref.~\cite{Laturia2018} for $\epsilon_\perp=2.91$. 
The spectrum of the excitons then reads $E_1\approx -228$\,meV, $E_2\approx -71$\,meV, $E_3\approx-35$\,meV, $E_4\approx-21$\,meV, $E_5\approx-14$\,meV.
It is surprisingly very close to the result of the homogeneous model, described in the main text, 
$E_1\approx-221$\,meV, $E_2\approx-70$\,meV, $E_3\approx-35$\,meV, $E_4\approx -21$\,meV, $E_5\approx -14$\,meV.
Therefore, we conclude that the homogeneous model provides a very good method for calculating the exciton spectrum, even in the case of an extremely thin top hBN flake of about 1-2 layers.

\section{Effective Coulomb potential in the S-TMD flake of finite thickness}
\label{app:vacuum_potential}

We consider a suspended multilayer  crystal of S-TMD as a set of $N$ layers of S-TMD, arranged in parallel to the $xy$ plane.
The position of $j$-th layer is defined by the coordinate $z_j$. We arrange the layers in the following way $0<z_1<z_2<\dots z_N<L$.
As in the previous case, we suppose that a multilayer is polarized in the in-plane direction, with the 2D susceptibility
$\chi_\text{TMD}=r_0/2\pi$. The out-of-plane polarization of the S-TMD crystal is $\epsilon_\perp$.

The electric potential $\Phi(\boldsymbol{\rho},z)$ for the point-like charge $Q$ at the point $\mathbf{r}=(0,0,z')$ of multilayer reads 
\begin{align}
\Big[\Delta_\parallel+\epsilon_\perp\frac{d^2}{dz^2}\Big]\Phi(\boldsymbol{\rho},z)=
&-4\pi Q\delta(\boldsymbol{\rho})\delta(z-z')-\nonumber \\ 
-&2r_0\sum_{j=1}^N \delta(z-z_j)\Delta_\parallel\Phi(\boldsymbol{\rho},z_j).
\end{align}
This equation can be solved with the help of Fourier transform
\begin{align}
\label{Fourier_transform}
\Phi(\boldsymbol{\rho},z)=\frac{1}{(2\pi)^3}\int d^2\mathbf{k}\int_{-\infty}^\infty dq\, e^{i\mathbf{k}\boldsymbol{\rho}+iqz}
\Phi(\mathbf{k},q).
\end{align}
After substitution it into the main equation one gets
\begin{equation}
\label{eq:non_linear_equation}
[k^2+\epsilon_\perp q^2]\Phi(\mathbf{k},q)=4\pi Qe^{-iqz'} -2r_0 k^2
\sum_{j=1}^N e^{-iqz_j}\Phi(\mathbf{k},z_j),
\end{equation}
where 
\begin{equation}
\Phi(\mathbf{k},z_j)=\frac{1}{2\pi}\int_{-\infty}^\infty dq e^{iqz_j}\Phi(\mathbf{k},q).
\end{equation}
Note that a solution of this equation can be found in the $N\rightarrow \infty$ limit, $i.e.$, the case of the infinite (bulk) S-TMD crystal. To do it we rewrite the finite sum in the equation in the form 
\begin{align}
\lim_{N\rightarrow \infty}\sum_{j=1}^N e^{-iqz_j}\Phi(\mathbf{k},z_j)=\frac{1}{d}\Phi(\mathbf{k},q).
\end{align}
Here, we used the parametrization $z_j=A + d (j-1)$ with $d=(B-A)/(N-1)$, with $A/B$ as the coordinate of the bottom/top layer of the multilayer, $d$ is the distance between layers in the crystal. To obtain the aforementioned result we present the sum in the form 
\begin{align}
\sum_{j=1}^N e^{i(q'-q)z_j}=e^{i(q'-q)\frac{(B+A)}{2}}
\frac{\sin\Big[\frac{(q'-q)}{2}dN\Big]}{\sin\Big[\frac{(q'-q)}{2}d\Big]},
\end{align}
then considering $(q'-q)dN/2\sim 1$, $(q'-q)d/2\sim 1/N$,  and using     
\begin{align}
\lim_{N\rightarrow \infty}\frac{\sin\Big[\frac{(q'-q)}{2}dN\Big]}{\Big[\frac{(q'-q)}{2}d\Big]}=
\pi\delta\Big[\frac{(q'-q)}{2}d\Big],
\end{align}
we obtain 
\begin{align}
\lim_{N\rightarrow \infty}\sum_{j=1}^N e^{i(q'-q)z_j}=\pi \delta\Big[\frac{(q'-q)}{2}d\Big].
\end{align}
Then one can rewrite the Eq.~(\ref{eq:non_linear_equation}) in the form 
\begin{equation}
\Big[\Big(1+2\frac{r_0}{d}\Big)k^2+\epsilon_\perp q^2\Big]\Phi(\mathbf{k},q)=4\pi Qe^{-iqz'}.
\end{equation}
This result coincides with the equation for the potential of charge $Q$, placed in the point $z'$ for the crystal
with the in-plane $\varepsilon_\parallel=1+2r_0/d$ and out-of-plane $\varepsilon_\perp=\epsilon_\perp$ 
dielectric constants, see \cite{Berkelbach2013}.  
 
To find the solution of Eq.~(\ref{eq:non_linear_equation}) for the finite number of layers $N$ we divide it on $[\mathbf{k}^2+\epsilon_\perp q^2]$, integrate over $q$ with additional $e^{iqz_m}$ function, evaluate the integral
\begin{equation}
\label{funny_integral}
\int_{-\infty}^\infty dq\frac{e^{iqz}}{k^2+\epsilon_\perp q^2}=\frac{\pi}{k\sqrt{\epsilon_\perp}}e^{-k|z|/\sqrt{\epsilon_\perp}}.
\end{equation}
and obtain the following system of equations for variables $\Phi(\mathbf{k},z_j)$
\begin{equation}
\sum_{j=1}^N \left[\delta_{mj}+\frac{kr_0}{\sqrt{\epsilon_\perp}}e^{-k\frac{|z_m-z_j|}{\sqrt{\epsilon_\perp}}}\right]\Phi(\mathbf{k},z_j)=\frac{2\pi Q}{k\sqrt{\epsilon_\perp}}e^{-k\frac{|z_m-z'|}{\sqrt{\epsilon_\perp}}}.
\end{equation}
This system of the linear equation can be solved analytically for small values of the number of layers $N \sim 1$. 
The solution for the larger numbers $N\gg 1$ can be done numerically. The obtained expressions for the potentials 
in the $z_j$th layer $\Phi(\mathbf{k},z_j)$ are needed to evaluate the effective Coulomb interaction between the electron
and hole localized in the corresponding layers, see Ref.~\cite{Kipczak2022}. 

The alternative way to find the solution of Eq.~(\ref{eq:non_linear_equation}) is to present it in the form of an integral equation
\begin{align}
\Phi(\mathbf{k},q)=\frac{2\pi Q e^{-iqz'}}{k^2+\epsilon_\perp q^2}-
\int_{-\infty}^\infty dq' f(q,q')\Phi(\mathbf{k},q'), 
\end{align}
with the kernel 
\begin{equation}
f(q,q')=\frac{r_0k^2}{k^2+\epsilon_\perp q^2}\frac{1}{\pi}\sum_{j=1}^N e^{-i(q-q')z_j},
\end{equation}
valid for any distribution of the coordinates $z_j$. 

\section{Spectrum of excitons for the different cases of the substrate} 

We evaluate the energy spectrum of excitons in the investigated structure for the case of different substrates as a function of the parameter $l$. 
The eigenvalues equation reads
\begin{align}
\Big[b^2\frac{1}{\xi}\frac{d}{d\xi}\Big(\xi\frac{d}{d\xi}\Big)+2b\phi(\xi,l,\varepsilon_1)+\epsilon\Big]\psi(\xi)=0,
\end{align}    
where we introduced $b=\hbar^2\varepsilon_\text{hBN}^2/(\mu e^2r_0)$ and $E=Ry^*\epsilon$ with 
$Ry^*=\mu e^4/(2\hbar^2\varepsilon_\text{hBN}^2)$, as in the main text. Here $\psi(\xi)$ represents the wave function of an exciton in
terms of dimensionless coordinate $\xi=\rho\varepsilon_\text{hBN}/r_0$.
The dimensionless potential function $\phi(\xi,l,\varepsilon_1)$ has a form 
\begin{widetext}
    \begin{align}
\phi(\xi,l,\varepsilon_1)=\int_0^\infty dx\frac{J_0(x\xi)\Big[1+\frac{\varepsilon_\text{hBN}-1}{\varepsilon_\text{hBN}+1}
\exp\Big(-2\sqrt{\frac{\varepsilon_{\text{hBN},\parallel}}{\varepsilon_{\text{hBN},\perp}}}xl\Big)\Big]}{
x+\frac{\varepsilon_\text{hBN}+\varepsilon_1}{2\varepsilon_\text{hBN}}+\Big[x+ \frac{\varepsilon_1-\varepsilon_\text{hBN}}
{2\varepsilon_\text{hBN}}\Big]\frac{\varepsilon_\text{hBN}-1}{\varepsilon_\text{hBN}+1}
\exp\Big(-2\sqrt{\frac{\varepsilon_{\text{hBN},\parallel}}{\varepsilon_{\text{hBN},\perp}}}xl\Big)}.
\end{align}
\end{widetext}
As one can see for $\varepsilon_1=\varepsilon_\text{hBN}$, it coincides with the previously obtained result, $i.e.$, $\phi(\xi,l,\varepsilon_\text{hBN})=\phi(\xi,l)$, as should be.

\begin{figure}[!t]
	\centering
	\includegraphics[width=1\linewidth]{spectrum_sio2_new.pdf}%
	\caption{Energy spectrum of $s$ excitonic state in the WSe$_2$ ML deposited on SiO$_2$ substrate and covered with top hBN layer as a function of its thickness. 
                The gray-shaded region represents the infinity of states above the bandgap energy.} 
	\label{fig:spectrum_sio2}
\end{figure}

\begin{center}
\begin{table}[!t]
\centering
\caption{Calculated binding energies of excitons ($E_\mathrm{b}$) in the WSe$_2$ ML placed on the SiO$_2$ substrate and covered with top hBN layer for selected numbers of the top hBN layer.}
\label{tab:spectrum_sio2}
\begin{tabular}{ccccccccc}
 \hline\hline %[-1.5ex]
 Number of \\ top hBN layers & 0 & 3 & 6 & 10 & 20 & 40 & 100 & $\infty$  \\ %[1.5ex]
 \hline 
  $E_\mathrm{b}$ (meV) & 386 & 310 & 281 & 263 & 245 & 234 & 226 & 220 \\ %[2.0ex]
 \hline  
 \end{tabular}
\end{table}
\end{center}

\begin{figure}[!t]
	\centering
	\includegraphics[width=1\linewidth]{spectrum_suspended_new.pdf}%
	\caption{Energy spectrum of $s$ excitonic state in the suspended WSe$_2$ ML covered with top hBN layer as a function of its thickness. 
                The gray-shaded region represents the infinity of states above the bandgap energy.} 
	\label{fig:spectrum_suspended}
\end{figure}

\begin{center}
\begin{table}[!t]
\centering
\caption{Calculated binding energies of excitons ($E_\mathrm{b}$) in the suspended WSe$_2$ ML covered with top hBN layer for selected numbers of the top hBN layer.}
\label{tab:spectrum_suspended}
\begin{tabular}{ccccccccc}
 \hline\hline %[-1.5ex]
 Number of \\ top hBN layers & 0 & 3 & 6 & 10 & 20 & 40 & 100 & $\infty$  \\ %[1.5ex]
 \hline 
  $E_\mathrm{b}$ (meV) & 499 & 391 & 350 & 324 & 296 & 278 & 266 & 256 \\ %[2.0ex]
 \hline  
 \end{tabular}
\end{table}
\end{center}

We solve the eigenvalue equation for the case of SiO$_2$ substrate, $\varepsilon_1=2.1$ \cite{Stier2016} 
and for the case of suspended S-TMD monolayer, $\varepsilon_1=1$.
The calculated energy spectra of an exciton for the ground (1$s$) and four excited (2$s$ $-$ 5$s$) states as a function of the thickness of the top hBN layer for the case of the SiO$_2$ substrate and of the suspended S-TMD monolayer are shown in Figs.~\ref{fig:spectrum_sio2} and \ref{fig:spectrum_suspended}, respectively.
The corresponding dependences of the excitonic binding energy ($E_b$, defined as the energy difference between the electronic bang gap and the ground 1$s$ state) in the WSe$_2$ ML for the case of the SiO$_2$ substrate and of the suspended S-TMD monolayer are summarized Tables~\ref{tab:spectrum_sio2} and \ref{tab:spectrum_suspended}.


\section{Spectrum of excitons for the case of the non-zero distance between monolayer and sub- and superstrate} 

Let us consider the general case of the S-TMD monolayer encapsulated in between different media, presented in Fig.~3 of the main text. 
In this scenario the $k$-depended, and, hence, $\rho$-dependent, effective in-plane Coulomb potential depends on three
distance parameters: the screening length in the plane of the S-TMD monolayer $r_0$, the thickness of the top flake $L$, 
and the distance $\delta$ between the monolayer and the substrate (the same distance is between the monolayer and the top flake). 
As a result, the shape of the Coulomb potential is modified, providing the three-parametric spectrum and wave functions of the
excitons. 
It makes their general analytical consideration quite tricky. 
However, some conclusions can be made 
by studying the limit cases $\delta\rightarrow 0$, $\delta\rightarrow \infty$, $L\rightarrow 0$, etc.

The limit $\delta\rightarrow 0$ is considered in the main text, where it was demonstrated that the spectrum depends on the
dimensionless parameter $L/r_0$. One can conclude that a similar answer can be obtained for small $\delta\ll r_0,L$.
The typical scale of binding energies of the excitons $E_\text{b}$ is suppressed by the dielectric constants of the surrounding media:
$E_\text{b}\propto Ry/(\varepsilon_1+\varepsilon_3)^2$ for $L\rightarrow 0$, and
$E_\text{b}\propto Ry/(\varepsilon_1+\varepsilon_2)^2$ for $L\rightarrow \infty$, see Ref.~\cite{Molas2019} for details.
The opposite limit $\delta\rightarrow\infty$ corresponds to the case of the suspended monolayer, with the dielectric function
$\varepsilon(k)=kr_0+1$. Therefore, the scale of the binding energies of excitons is $E_\text{b}\propto Ry$. 
The intermediate case, where $\delta \sim r_0,L$, interpolates between the two aforementioned limits. Therefore, for fixed parameters
$r_0,L$, the binding energies are increasing with the increasing $\delta$, see also Ref.~\cite{Florian2018}.

In order to demonstrate the impact of this parameter on the excitons' spectrum in such a system, we consider the 
WSe$_2$ monolayer, encapsulated in hBN medium, with $\delta=5\,\mbox{\AA}$, as an example.
The corresponding eigenvalue equation has a form 
\begin{align}
\Big[b^2\frac{1}{\xi}\frac{d}{d\xi}\Big(\xi\frac{d}{d\xi}\Big)+2b\phi(\xi,l,\eta)+\epsilon\Big]\psi(\xi)=0,
\end{align}    
where $l=\varepsilon_\text{hBN} L/r_0$, $\eta=\varepsilon_\text{hBN}\delta/r_0$,
$b=\hbar^2\varepsilon_\text{hBN}^2/(\mu e^2r_0)$, $E=Ry^*\epsilon$,
$Ry^*=\mu e^4/(2\hbar^2\varepsilon_\text{hBN}^2)$.
The dimensionless potential function has a form 
\begin{equation}
\phi(\xi,l,\eta)=\int_0^\infty dx J_0(x\xi)/\varepsilon(x,l,\eta),
\end{equation}
with the $\eta$-dependent dielectric function
\begin{widetext}
\begin{align}
\varepsilon(x,l,\eta)=x+
\frac{1-\alpha^2\exp[-4x\eta]-\alpha^2(1-\exp[-4x\eta])
\exp\big[-2\sqrt{\frac{\varepsilon_{\text{hBN},\parallel}}{\varepsilon_{\text{hBN},\perp}}} x(l-\eta)\big]}{\varepsilon_\text{hBN}(1-\alpha \exp[-2x\eta])(1-\alpha \exp[-2x\eta]+\alpha(\exp[-2x\eta]-\alpha)\exp\big[-2\sqrt{\frac{\varepsilon_{\text{hBN},\parallel}}{\varepsilon_{\text{hBN},\perp}}} x(l-\eta)\big])},
\end{align}
\end{widetext}
and $\alpha=(\varepsilon_\text{hBN}-1)/(\varepsilon_\text{hBN}+1)$.
The calculated spectrum, as a function of the number of the layers of the top hBN layer, is presented in Fig.~\ref{fig:spectrum_nonzero}.
The corresponding dependence of the $E_b$ energy is summarized Table~\ref{tab:spectrum_nonzero}.

\begin{figure}[!t]
	\centering
	\includegraphics[width=1\linewidth]{spectrum_nonzero.pdf}%
	\caption{Energy spectrum of $s$ excitonic state in the hBN-encapsulated WSe$_2$ ML covered with top hBN layer as a function of its thickness for the non-zero distance, $\delta=5\,\mbox{\AA}$, between the ML and sub- and superstrate. 
                The gray-shaded region represents the infinity of states above the bandgap energy.} 
	\label{fig:spectrum_nonzero}
\end{figure}

\begin{center}
\begin{table}[!h]
\centering
\caption{Calculated binding energies of excitons ($E_\mathrm{b}$) in the hBN-encapsulated  WSe$_2$ ML covered with top hBN layer as a function of the number of layers of the top hBN layer for the non-zero distance between the ML and sub- and superstrate, $\delta=5\,\mbox{\AA}$.}
\label{tab:spectrum_nonzero}
\begin{tabular}{ccccccccc}
 \hline\hline %[-1.5ex]
 Number of \\ top hBN layers & 0 & 3 & 6 & 10 & 20 & 40 & 100 & $\infty$  \\ %[1.5ex]
 \hline 
  $E_\mathrm{b}$ (meV) & 336 & 284 & 274 & 270 & 267 & 266 & 265 & 265 \\ %[2.0ex]
 \hline  
 \end{tabular}
\end{table}
\end{center}

One can see that the obtained excitonic ladder for the relatively large parameter $\delta$ deviates significantly from the ladder obtained in the main text ($\delta=0$). 
This conclusion is valid also for the general case, presented in Fig.~3 of the main text.
It provides us with the instrument for the analysis of the spectrum in realistic heterostructures. 
Namely, knowing the parameters of the system, one can first calculate the spectrum for the case of $\delta=0$ 
(provided in the main text). If the calculated spectrum significantly deviates from the experimentally observed excitonic ladder, one concludes that there is a non-zero distance gap between the layers, and the more general model, with $\delta>0$, should be considered. 





